Convergence for score-based generative modeling with polynomial complexity

Score-based generative modeling (SGM) is a highly successful approach for learning a probability distribution from data and generating further samples. We prove the first polynomial convergence guarantees for the core mechanic behind SGM: drawing samples from a probability density $p$ given a score estimate (an estimate of $\nabla \ln p$) that is accurate in $L^2(p)$. Compared to previous works, we do not incur error that grows exponentially in time or that suffers from a curse of dimensionality. Our guarantee works for any smooth distribution and depends polynomially on its log-Sobolev constant. Using our guarantee, we give a theoretical analysis of score-based generative modeling, which transforms white-noise input into samples from a learned data distribution given score estimates at different noise scales. Our analysis gives theoretical grounding to the observation that an annealed procedure is required in practice to generate good samples, as our proof depends essentially on using annealing to obtain a warm start at each step. Moreover, we show that a predictor-corrector algorithm gives better convergence than using either portion alone.

==> checklist.tex <==
\begin{enumerate}
\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \textcolor{blue}{[Yes]}  
  \item Did you describe the limitations of your work?
    \textcolor{blue}{[Yes]}
  \item Did you discuss any potential negative societal impacts of your work?
   \answerNA{}
    %\textcolor{blue}{[Yes]}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \textcolor{blue}{[Yes]}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \textcolor{blue}{[Yes]}
        \item Did you include complete proofs of all theoretical results?
    \textcolor{blue}{[Yes]}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerNA{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerNA{}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNA{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNA{}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerNA{}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}


==> neurips.tex <==
% \documentclass{article}
% \usepackage[utf8]{inputenc}


% % if you need to pass options to natbib, use, e.g.:
% %     \PassOptionsToPackage{numbers, compress}{natbib}
% % before loading neurips_2022


% % ready for submission
% \usepackage[nonatbib,final]{neurips_2022}


% % to compile a preprint version, e.g., for submission to arXiv, add add the
% % [preprint] option:
% %     \usepackage[preprint]{neurips_2022}


% % to compile a camera-ready version, add the [final] option, e.g.:
% %     \usepackage[final]{neurips_2022}


% % to avoid loading the natbib package, add option nonatbib:
% %    \usepackage[nonatbib]{neurips_2022}


% % \usepackage[utf8]{inputenc} % allow utf-8 input
% % \usepackage[T1]{fontenc}    % use 8-bit T1 fonts
% % \usepackage{hyperref}       % hyperlinks
% % \usepackage{url}            % simple URL typesetting
% % \usepackage{booktabs}       % professional-quality tables
% % \usepackage{amsfonts}       % blackboard math symbols
% % \usepackage{nicefrac}       % compact symbols for 1/2, etc.
% % \usepackage{microtype}      % microtypography
% % \usepackage{xcolor}         % colors
% \input{macros}
% \input{packages-neurips}
% \input{theorems}
% \addbibresource{bib.bib}
% \usepackage{xcolor}         % colors
% \renewcommand{\answerYes}[1][]{\textcolor{blue}{[Yes] #1}}
% \renewcommand{\answerNo}[1][]{\textcolor{orange}{[No] #1}}
% \renewcommand{\answerNA}[1][]{\textcolor{gray}{[N/A] #1}}
% \renewcommand{\answerTODO}[1][]{\textcolor{red}{\bf [TODO]}}
% \title{Convergence for score-based generative modeling with polynomial complexity}


% % The \author macro works with any number of authors. There are two commands
% % used to separate the names and addresses of multiple authors: \And and \AND.
% %
% % Using \And between authors leaves it to LaTeX to determine where to break the
% % lines. Using \AND forces a line break at that point. So, if LaTeX puts 3 of 4
% % authors names on the first line, and the last on the second line, try using
% % \AND instead of \And before the third author name.


% \author{%
%     Holden Lee%\quad Jianfeng Lu\quad Yixin Tan
%     \\
%   Department of Applied Mathematics and Statistics\\
%   Johns Hopkins University\\
%  %Durham, NC 27708 \\
%   \texttt{hlee283@jhu.edu}%\quad \texttt{jianfeng@math.duke.edu \quad \texttt{yixin.tan@duke.edu}} \\
%   \And
%     Jianfeng Lu\\
%   Department of Mathematics\\
%   Duke University\\
%  %Durham, NC 27708 \\
%   \texttt{jianfeng@math.duke.edu} \\
%   \And
%   Yixin Tan\\
%   Department of Mathematics\\
%   Duke University\\
%  %Durham, NC 27708 \\
%   \texttt{yixin.tan@duke.edu} \\
%   % examples of more authors
%   % \And
%   % Coauthor \\
%   % Affiliation \\
%   % Address \\
%   % \texttt{email} \\
%   % \AND
%   % Coauthor \\
%   % Affiliation \\
%   % Address \\
%   % \texttt{email} \\
%   % \And
%   % Coauthor \\
%   % Affiliation \\
%   % Address \\
%   % \texttt{email} \\
%   % \And
%   % Coauthor \\
%   % Affiliation \\
%   % Address \\
%   % \texttt{email} \\
% }



% \begin{document}

% \input{macros2}


% \maketitle

% \input{abstract}

% %\fixme{[A few mistakes, marked in red, have been corrected in the main text.]} 
% \input{introduction}

% %HL: moved to separate file and to appendix
% %\input{predictor}

% \input{results-corrector}
% \input{results-predictor}
% \input{sketch}
% \input{conclusion}
% \input{acknowledgement}

% \newpage

% %\bibliography{bib}
% \printbibliography

% \newpage 

% \input{checklist}

% \newpage

% %\input{notations}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% \appendix

% \input{calcs}
% \input{corrector}
% \input{predictor}
% \input{counterex}
% \input{facts}

% %Better bounds for section C, swap in for revision
% %\input{holden}


% \end{document}

==> notations.tex <==
\fixme{
Notation:
\begin{itemize}
    \item $\smf,\sms$ for smoothness (change from $\be_f,\be_s$)
    \item $V$ for potential (change from $f$)
    \item $P$ for measure, $p$ for density (change from just using $p$)
    \item Discretized process: $p_{nh}$ (change from $p_n$)
    \item Forward process $\Tilde p_t$.
    \item Discretized (and interpolated) process: $q_t$.
    \item Hypothetical process for comparison $\ol q_t$.
    \item SDE's: lowercase letters.
    \item Noise levels $1\le m\le M$.
    \item $p_{\si^2} = \ph* g_{\si^2}$.
    \item $\chi^2(q||p)$ and $\KL(q||p)$ (with 2 bars).
    \item iteration index $m$ or $k$?
    \item $C_T$ for log-Sobolev constant vs. ratio of time
\end{itemize}
}


==> packages-neurips.tex <==


\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{mathrsfs}
\usepackage{bbm}
\usepackage{cancel}
\usepackage{hyperref}
\usepackage{thm-restate}
\usepackage{xypic}
%https://www.jmilne.org/not/Mxymatrix.pdf

\usepackage{algorithm}
\usepackage{algorithmicx,algpseudocode}
\usepackage{titleref}

\usepackage{color}

\usepackage[backend=biber,style=alphabetic,maxbibnames=99]{biblatex}
